A Systematic Study on the Resonance in Collisional Neutrino Flavor Instability

Investigations on the resonance in the collisional flavor instability (CFI) of neutrinos, which were reported recently, are reported. We show that the resonance occurs not only for the isotropy-preserving modes as pointed out in the previous work but also for the isotropy-breaking modes and that it enhances the growth rate of CFI by orders of magnitude. Employing the linear analysis and nonlinear numerical simulations in the two-flavor scheme and under the relaxation approximation for the collision term, we discuss the criterion for the resonance, its effect on the nonlinear evolution as well as the influences of homogeneity-breaking (k \ne 0) perturbations as well as of anisotropy in the background on the resonance. We will also touch the cohabitation of the resonance with the fast flavor conversion (FFC).

==> apssamp.tex <==
@PREAMBLE{
	"\providecommand{\noopsort}[1]{}" 
	# "\providecommand{\singleletter}[1]{#1}%" 
}

@article{Airen_2018,
	doi = {10.1088/1475-7516/2018/12/019},
	url = {https://dx.doi.org/10.1088/1475-7516/2018/12/019},
	year = {2018},
	month = {dec},
	publisher = {},
	volume = {2018},
	number = {12},
	pages = {019},
	author = {Sagar Airen and Francesco Capozzi and Sovan Chakraborty and Basudeb Dasgupta and Georg Raffelt and Tobias Stirner},
	title = {Normal-mode analysis for collective neutrino oscillations},
	journal = {Journal of Cosmology and Astroparticle Physics},
	abstract = {In an interacting neutrino gas, collective modes of flavor coherence emerge that can be propagating or unstable. We derive the general dispersion relation in the linear regime that depends on the neutrino energy and angle distribution. The essential scales are the vacuum oscillation frequency ω=Δ m2/(2E), the neutrino-neutrino interaction energy μ=√2GF; nν, and the matter potential λ=√2GF ne. Collective modes require non-vanishing μ and may be dynamical even for ω=0 (“fast modes”), or they may require ω¬=0 (“slow modes”). The growth rate of unstable fast modes can be fast itself (independent of ω) or can be slow (suppressed by √|ω/μ|). We clarify the role of flavor mixing, which is ignored for the identification of collective modes, but necessary to trigger collective flavor motion. A large matter effect is needed to provide an approximate fixed point of flavor evolution, while spatial or temporal variations of matter and/or neutrinos are required as a trigger, i.e., to translate the disturbance provided by the mass term to seed stable or unstable flavor waves. We work out explicit examples to illustrate these points.}
}

@article{PhysRevLett.118.021101,
	title = {Fast Pairwise Conversion of Supernova Neutrinos: A Dispersion Relation Approach},
	author = {Izaguirre, Ignacio and Raffelt, Georg and Tamborra, Irene},
	journal = {Phys. Rev. Lett.},
	volume = {118},
	issue = {2},
	pages = {021101},
	numpages = {6},
	year = {2017},
	month = {Jan},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevLett.118.021101},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.118.021101}
}

@misc{luke2019,
	doi = {10.48550/ARXIV.2104.11369},
	
	url = {https://arxiv.org/abs/2104.11369},
	
	author = {Johns, Lucas},
	
	keywords = {High Energy Physics - Phenomenology (hep-ph), High Energy Astrophysical Phenomena (astro-ph.HE), FOS: Physical sciences, FOS: Physical sciences},
	
	title = {Collisional flavor instabilities of supernova neutrinos},
	
	publisher = {arXiv},
	
	year = {2021},
	
	copyright = {arXiv.org perpetual, non-exclusive license}
}

@misc{duan,
	doi = {10.48550/ARXIV.2210.09218},
	
	url = {https://arxiv.org/abs/2210.09218},
	
	author = {Lin, Yu-Chia and Duan, Huaiyu},
	
	keywords = {High Energy Physics - Phenomenology (hep-ph), High Energy Astrophysical Phenomena (astro-ph.HE), Nuclear Theory (nucl-th), FOS: Physical sciences, FOS: Physical sciences},
	
	title = {Collision-induced flavor instability in dense neutrino gases with energy-dependent scattering},
	
	publisher = {arXiv},
	
	year = {2022},
	
	copyright = {arXiv.org perpetual, non-exclusive license}
}

@misc{2022,
	doi = {10.48550/ARXIV.2212.03750},
	
	url = {https://arxiv.org/abs/2212.03750},
	
	author = {Xiong, Zewei and Johns, Lucas and Wu, Meng-Ru and Duan, Huaiyu},
	
	keywords = {High Energy Physics - Phenomenology (hep-ph), High Energy Astrophysical Phenomena (astro-ph.HE), Nuclear Theory (nucl-th), FOS: Physical sciences, FOS: Physical sciences},
	
	title = {Collisional flavor instability in dense neutrino gases},
	
	publisher = {arXiv},
	
	year = {2022},
	
	copyright = {arXiv.org perpetual, non-exclusive license}
}

@ARTICLE{finalstate,
	author = {{Zaizen}, Masamichi and {Nagakura}, Hiroki},
	title = "{Simple method for determining asymptotic states of fast neutrino-flavor conversion}",
	journal = {arXiv e-prints},
	keywords = {Astrophysics - High Energy Astrophysical Phenomena, High Energy Physics - Phenomenology},
	year = 2022,
	month = nov,
	eid = {arXiv:2211.09343},
	pages = {arXiv:2211.09343},
	archivePrefix = {arXiv},
	eprint = {2211.09343},
	primaryClass = {astro-ph.HE},
	adsurl = {https://ui.adsabs.harvard.edu/abs/2022arXiv221109343Z},
	adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{PhysRevD.103.063002,
	title = {Change of direction in pairwise neutrino conversion physics: The effect of collisions},
	author = {Shalgar, Shashank and Tamborra, Irene},
	journal = {Phys. Rev. D},
	volume = {103},
	issue = {6},
	pages = {063002},
	numpages = {11},
	year = {2021},
	month = {Mar},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevD.103.063002},
	url = {https://link.aps.org/doi/10.1103/PhysRevD.103.063002}
}

@article{PhysRevLett.122.091101,
	title = {Collisional Triggering of Fast Flavor Conversions of Supernova Neutrinos},
	author = {Capozzi, Francesco and Dasgupta, Basudeb and Mirizzi, Alessandro and Sen, Manibrata and Sigl, G\"unter},
	journal = {Phys. Rev. Lett.},
	volume = {122},
	issue = {9},
	pages = {091101},
	numpages = {6},
	year = {2019},
	month = {Mar},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevLett.122.091101},
	url = {https://link.aps.org/doi/10.1103/PhysRevLett.122.091101}
}

@article{PhysRevD.106.103029,
	title = {Collisional instabilities of neutrinos and their interplay with fast flavor conversion in compact objects},
	author = {Johns, Lucas and Xiong, Zewei},
	journal = {Phys. Rev. D},
	volume = {106},
	issue = {10},
	pages = {103029},
	numpages = {13},
	year = {2022},
	month = {Nov},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevD.106.103029},
	url = {https://link.aps.org/doi/10.1103/PhysRevD.106.103029}
}

@article{Shalgar_2019,
	doi = {10.3847/1538-4357/ab38ba},
	url = {https://dx.doi.org/10.3847/1538-4357/ab38ba},
	year = {2019},
	month = {sep},
	publisher = {The American Astronomical Society},
	volume = {883},
	number = {1},
	pages = {80},
	author = {Shashank Shalgar and Irene Tamborra},
	title = {On the Occurrence of Crossings between the Angular Distributions of Electron Neutrinos and Antineutrinos in the Supernova Core},
	journal = {The Astrophysical Journal},
	abstract = {Neutrino fast pairwise conversions have been postulated to occur in the dense core of a core-collapse supernova (SN), possibly having dramatic consequences on the SN mechanism and the observable neutrino signal. One crucial condition favoring pairwise conversions is the presence of crossings between the electron neutrino and antineutrino angular distributions (i.e., electron neutrino lepton number crossings, ELN crossings). A stationary and spherically symmetric SN toy model is constructed to reproduce the development of the neutrino angular distributions in the dense SN core in the absence of perturbations induced by hydrodynamical instabilities. By iteratively solving the neutrino Boltzmann equations including the collisional term, our model predicts that ELN crossings can develop only in the proximity of the decoupling region and for a sharp radial evolution of the baryon density, when the electron neutrino and antineutrino number densities are comparable. Such conditions are likely to occur only in the late SN stages. Interestingly, flavor instabilities induced by spatial or temporal perturbations are unlikely to generate ELN crossings dynamically within our simplified setup.}
}

@article{PhysRevD.103.063001,
	title = {Fast flavor oscillations in dense neutrino media with collisions},
	author = {Martin, Joshua D. and Carlson, J. and Cirigliano, Vincenzo and Duan, Huaiyu},
	journal = {Phys. Rev. D},
	volume = {103},
	issue = {6},
	pages = {063001},
	numpages = {13},
	year = {2021},
	month = {Mar},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevD.103.063001},
	url = {https://link.aps.org/doi/10.1103/PhysRevD.103.063001}
}

@article{PhysRevD.105.043005,
	title = {Simulations of fast neutrino flavor conversions with interactions in inhomogeneous media},
	author = {Sigl, G\"unter},
	journal = {Phys. Rev. D},
	volume = {105},
	issue = {4},
	pages = {043005},
	numpages = {18},
	year = {2022},
	month = {Feb},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevD.105.043005},
	url = {https://link.aps.org/doi/10.1103/PhysRevD.105.043005}
}

@article{Kato_2021,
	doi = {10.3847/1538-4365/ac2aa4},
	url = {https://dx.doi.org/10.3847/1538-4365/ac2aa4},
	year = {2021},
	month = {dec},
	publisher = {The American Astronomical Society},
	volume = {257},
	number = {2},
	pages = {55},
	author = {Chinami Kato and Hiroki Nagakura and Taiki Morinaga},
	title = {Neutrino Transport with the Monte Carlo Method. II. Quantum Kinetic Equations},
	journal = {The Astrophysical Journal Supplement Series},
	abstract = {Neutrinos have a unique quantum feature as flavor conversions. Recent studies suggested that collective neutrino oscillations play important roles in high-energy astrophysical phenomena. The quantum kinetic equation (QKE) is capable of describing the neutrino flavor conversion, transport, and matter collision self-consistently. However, we have experienced many technical difficulties in their numerical implementation. In this paper, we present a new QKE solver based on a Monte Carlo (MC) approach. This is an upgraded version of our classical MC neutrino transport solver; in essence, a flavor degree of freedom including mixing state is added into each MC particle. This extension requires updating numerical treatments of collision terms, in particular for scattering processes. We deal with the technical problem by generating a new MC particle at each scattering event. To reduce statistical noise inherent in MC methods, we develop the effective mean free path method. This suppresses a sudden change of flavor state due to collisions without increasing the number of MC particles. We present a suite of code tests to validate these new modules with comparison to the results reported in previous studies. Our QKE-MC solver is developed with fundamentally different philosophy and design from other deterministic and mesh methods, suggesting that it will be complementary to others and potentially provide new insights into physical processes of neutrino dynamics.}
}

@article{10.1093/ptep/ptac082,
	author = {Sasaki, Hirokazu and Takiwaki, Tomoya},
	title = "{A detailed analysis of the dynamics of fast neutrino flavor conversions with scattering effects}",
	journal = {Progress of Theoretical and Experimental Physics},
	volume = {2022},
	number = {7},
	year = {2022},
	month = {06},
	abstract = "{We calculate the dynamics of fast neutrino flavor conversions with Boltzmann collisions of neutrino scatterings in a homogeneous system. We find the enhancement or suppression of the flavor conversions in various setups of the collision terms. We analyze the mechanism of fast flavor conversions based on the motion of polarization vectors in the cylindrical coordinate analogous to a pendulum motion. The phases of the all the polarization vectors synchronize in the linear evolution phase, and the phase deviation from the Hamiltonian governs the neutrino flavor conversions. In a non-linear regime of flavor conversions, the collision terms induce a spiral motion of the polarization vector and gradually make the phase space smaller. The collision terms align all of the polarization vectors, and the flavor conversions eventually settle into equilibrium when the distributions of neutrinos become isotropic. Though our current analysis does not fully clarify the non-linear phenomena of fast flavor conversions, the framework of the pendulum motion gives a new insight into this complicated phenomenon that will be helpful in further studies.}",
	issn = {2050-3911},
	doi = {10.1093/ptep/ptac082},
	url = {https://doi.org/10.1093/ptep/ptac082},
	note = {073E01},
	eprint = {https://academic.oup.com/ptep/article-pdf/2022/7/073E01/44400755/ptac082.pdf},
}

@article{PhysRevD.105.123003,
	title = {Enhancement or damping of fast neutrino flavor conversions due to collisions},
	author = {Hansen, Rasmus S. L. and Shalgar, Shashank and Tamborra, Irene},
	journal = {Phys. Rev. D},
	volume = {105},
	issue = {12},
	pages = {123003},
	numpages = {12},
	year = {2022},
	month = {Jun},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevD.105.123003},
	url = {https://link.aps.org/doi/10.1103/PhysRevD.105.123003}
}

@article{PhysRevD.106.043031,
	title = {Self-consistency in models of neutrino scattering and fast flavor conversion},
	author = {Johns, Lucas and Nagakura, Hiroki},
	journal = {Phys. Rev. D},
	volume = {106},
	issue = {4},
	pages = {043031},
	numpages = {11},
	year = {2022},
	month = {Aug},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevD.106.043031},
	url = {https://link.aps.org/doi/10.1103/PhysRevD.106.043031}
}

@misc{https://doi.org/10.48550/arxiv.2207.04058,
	doi = {10.48550/ARXIV.2207.04058},
	
	url = {https://arxiv.org/abs/2207.04058},
	
	author = {Shalgar, Shashank and Tamborra, Irene},
	
	keywords = {High Energy Astrophysical Phenomena (astro-ph.HE), High Energy Physics - Phenomenology (hep-ph), FOS: Physical sciences, FOS: Physical sciences},
	
	title = {Neutrino Flavor Conversion, Advection, and Collisions: The Full Solution},
	
	publisher = {arXiv},
	
	year = {2022},
	
	copyright = {arXiv.org perpetual, non-exclusive license}
}

@article{Kato_2022,
	doi = {10.1103/physrevd.106.123013},
	
	url = {https://doi.org/10.1103%2Fphysrevd.106.123013},
	
	year = 2022,
	month = {dec},
	
	publisher = {American Physical Society ({APS})},
	
	volume = {106},
	
	number = {12},
	
	author = {Chinami Kato and Hiroki Nagakura},
	
	title = {Effects of energy-dependent scatterings on fast neutrino flavor conversions},
	
	journal = {Physical Review D}
}

@article{PhysRevD.46.510,
	title = {Dirac neutrinos in dense matter},
	author = {Pantaleone, James},
	journal = {Phys. Rev. D},
	volume = {46},
	issue = {2},
	pages = {510--523},
	numpages = {0},
	year = {1992},
	month = {Jul},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevD.46.510},
	url = {https://link.aps.org/doi/10.1103/PhysRevD.46.510}
}

@article{Sigl1993GeneralKD,
	title={General kinetic description of relativistic mixed neutrinos},
	author={Gunter Sigl and Georg Raffelt},
	journal={Nuclear Physics},
	year={1993},
	volume={406},
	pages={423-451}
}

@article{doi:10.1146/annurev.nucl.012809.104524,
	author = {Duan, Huaiyu and Fuller, George M. and Qian, Yong-Zhong},
	title = {Collective Neutrino Oscillations},
	journal = {Annual Review of Nuclear and Particle Science},
	volume = {60},
	number = {1},
	pages = {569-594},
	year = {2010},
	doi = {10.1146/annurev.nucl.012809.104524},
	
	URL = { 
		
		https://doi.org/10.1146/annurev.nucl.012809.104524
		
		
		
	},
	eprint = { 
		
		https://doi.org/10.1146/annurev.nucl.012809.104524
		
		
		
	}
	,
	abstract = { We review the rich phenomena associated with neutrino flavor transformation in the presence of neutrino self-coupling. Our exposition centers on three collective neutrino oscillation scenarios: (a) a simple bipolar neutrino system that initially consists of monoenergetic νe and , (b) a homogeneous and isotropic neutrino gas with multiple neutrino/antineutrino species and continuous energy spectra, and (c) a generic neutrino gas in an anisotropic environment. We use each of these scenarios to illustrate key facets of collective neutrino oscillations. We discuss the implications of collective neutrino flavor oscillations for core-collapse supernova physics and for the prospects of obtaining and/or constraining fundamental neutrino properties, such as the neutrino mass hierarchy and θ13 from a future observed supernova neutrino signal. }
}

@article{CHAKRABORTY2016366,
	title = {Collective neutrino flavor conversion: Recent developments},
	journal = {Nuclear Physics B},
	volume = {908},
	pages = {366-381},
	year = {2016},
	note = {Neutrino Oscillations: Celebrating the Nobel Prize in Physics 2015},
	issn = {0550-3213},
	doi = {https://doi.org/10.1016/j.nuclphysb.2016.02.012},
	url = {https://www.sciencedirect.com/science/article/pii/S0550321316000560},
	author = {Sovan Chakraborty and Rasmus Hansen and Ignacio Izaguirre and Georg Raffelt},
	abstract = {Neutrino flavor evolution in core-collapse supernovae, neutron-star mergers, or the early universe is dominated by neutrino–neutrino refraction, often spawning “self-induced flavor conversion,” i.e., shuffling of flavor among momentum modes. This effect is driven by collective run-away modes of the coupled “flavor oscillators” and can spontaneously break the initial symmetries such as axial symmetry, homogeneity, isotropy, and even stationarity. Moreover, the growth rates of unstable modes can be of the order of the neutrino–neutrino interaction energy instead of the much smaller vacuum oscillation frequency: self-induced flavor conversion does not always require neutrino masses. We illustrate these newly found phenomena in terms of simple toy models. What happens in realistic astrophysical settings is up to speculation at present.}
}

@article{doi:10.1146/annurev-nucl-102920-050505,
	author = {Tamborra, Irene and Shalgar, Shashank},
	title = {New Developments in Flavor Evolution of a Dense Neutrino Gas},
	journal = {Annual Review of Nuclear and Particle Science},
	volume = {71},
	number = {1},
	pages = {165-188},
	year = {2021},
	doi = {10.1146/annurev-nucl-102920-050505},
	
	URL = { 
		
		https://doi.org/10.1146/annurev-nucl-102920-050505
		
		
		
	},
	eprint = { 
		
		https://doi.org/10.1146/annurev-nucl-102920-050505
		
		
		
	}
	,
	abstract = { Neutrino–neutrino refraction dominates the flavor evolution in core-collapse supernovae, neutron star mergers, and the early Universe. Ordinary neutrino flavor conversions develop on timescales determined by the vacuum oscillation frequency. However, when the neutrino density is large enough, collective flavor conversions may arise because of pairwise neutrino scattering. Pairwise conversions are deemed fast because they are expected to occur on timescales that depend on the neutrino–neutrino interaction energy (i.e., on the neutrino number density) and are regulated by the angular distributions of electron neutrinos and antineutrinos. The enigmatic phenomenon of fast pairwise conversions has been overlooked for a long time. However, because of the fast conversion rate, pairwise conversions could occur in the proximity of the neutrino decoupling region with yet-to-be-understood implications for the hydrodynamics of astrophysical sources and the synthesis of the heavy elements. We review the physics of this fascinating phenomenon and its implications for neutrino-dense sources. }
}

@misc{https://doi.org/10.48550/arxiv.2207.03561,
	doi = {10.48550/ARXIV.2207.03561},
	
	url = {https://arxiv.org/abs/2207.03561},
	
	author = {Richers, Sherwood and Sen, Manibrata},
	
	keywords = {High Energy Astrophysical Phenomena (astro-ph.HE), High Energy Physics - Phenomenology (hep-ph), FOS: Physical sciences, FOS: Physical sciences},
	
	title = {Fast Flavor Transformations},
	
	publisher = {arXiv},
	
	year = {2022},
	
	copyright = {Creative Commons Attribution 4.0 International}
}



%searching for crossing in CCSNe
@article{PhysRevD.100.043004,
	title = {On the occurrence of fast neutrino flavor conversions in multidimensional supernova models},
	author = {Abbar, Sajad and Duan, Huaiyu and Sumiyoshi, Kohsuke and Takiwaki, Tomoya and Volpe, Maria Cristina},
	journal = {Phys. Rev. D},
	volume = {100},
	issue = {4},
	pages = {043004},
	numpages = {7},
	year = {2019},
	month = {Aug},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevD.100.043004},
	url = {https://link.aps.org/doi/10.1103/PhysRevD.100.043004}
}

@article{Nagakura_2019,
	doi = {10.3847/1538-4357/ab4cf2},
	url = {https://dx.doi.org/10.3847/1538-4357/ab4cf2},
	year = {2019},
	month = {nov},
	publisher = {The American Astronomical Society},
	volume = {886},
	number = {2},
	pages = {139},
	author = {Hiroki Nagakura and Taiki Morinaga and Chinami Kato and Shoichi Yamada},
	title = {Fast-pairwise Collective Neutrino Oscillations Associated with Asymmetric Neutrino Emissions in Core-collapse Supernovae},
	journal = {The Astrophysical Journal},
	abstract = {We present a linear stability analysis of the fast-pairwise neutrino flavor conversion based on a result of our latest axisymmetric core-collapse supernova (CCSN) simulation with full Boltzmann neutrino transport. In the CCSN simulation, coherent asymmetric neutrino emissions of electron-type neutrinos (νe) and their antiparticles (), in which the asymmetries of νe and  are anticorrelated with each other, occur at almost the same time as the onset of aspherical shock expansion. We find that the asymmetric neutrino emissions play a crucial role on occurrences of fast flavor conversions. The linear analysis shows that unstable modes appear in both pre- and post-shock flows; for the latter, they appear only in the hemisphere of higher  emissions (the same hemisphere with stronger shock expansion). We analyze the characteristics of electron–lepton number (ELN) crossing in depth by closely inspecting the angular distributions of neutrinos in momentum space. The ELN crossing happens in various ways, and the property depends on the radius: in the vicinity of neutron star,  (νe) dominates over νe () in the forward (backward) direction; at the larger radius, the ELN crossing occurs in the opposite way. We also find that the non-radial ELN crossing occurs at the boundary between no ELN crossing and the radial one, which is an effect of genuine multi-dimensional transport. Our findings indicate that the collective neutrino oscillation may occur more commonly in CCSNe and suggest that the CCSN community needs to accommodate these oscillations self-consistently in the modeling of CCSNe.}
}

@article{PhysRevD.101.023018,
	title = {Fast collective neutrino oscillations inside the neutrino sphere in core-collapse supernovae},
	author = {Delfan Azari, Milad and Yamada, Shoichi and Morinaga, Taiki and Nagakura, Hiroki and Furusawa, Shun and Harada, Akira and Okawa, Hirotada and Iwakami, Wakana and Sumiyoshi, Kohsuke},
	journal = {Phys. Rev. D},
	volume = {101},
	issue = {2},
	pages = {023018},
	numpages = {12},
	year = {2020},
	month = {Jan},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevD.101.023018},
	url = {https://link.aps.org/doi/10.1103/PhysRevD.101.023018}
}

@article{PhysRevD.101.043016,
	title = {Fast neutrino flavor conversion modes in multidimensional core-collapse supernova models: The role of the asymmetric neutrino distributions},
	author = {Abbar, Sajad and Duan, Huaiyu and Sumiyoshi, Kohsuke and Takiwaki, Tomoya and Volpe, Maria Cristina},
	journal = {Phys. Rev. D},
	volume = {101},
	issue = {4},
	pages = {043016},
	numpages = {12},
	year = {2020},
	month = {Feb},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevD.101.043016},
	url = {https://link.aps.org/doi/10.1103/PhysRevD.101.043016}
}

@article{PhysRevResearch.2.012046,
	title = {Fast neutrino-flavor conversion in the preshock region of core-collapse supernovae},
	author = {Morinaga, Taiki and Nagakura, Hiroki and Kato, Chinami and Yamada, Shoichi},
	journal = {Phys. Rev. Res.},
	volume = {2},
	issue = {1},
	pages = {012046},
	numpages = {6},
	year = {2020},
	month = {Feb},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevResearch.2.012046},
	url = {https://link.aps.org/doi/10.1103/PhysRevResearch.2.012046}
}

@article{PhysRevD.101.063001,
	title = {Fast neutrino flavor instability in the neutron-star convection layer of three-dimensional supernova models},
	author = {Glas, Robert and Janka, H.-Thomas and Capozzi, Francesco and Sen, Manibrata and Dasgupta, Basudeb and Mirizzi, Alessandro and Sigl, G\"unter},
	journal = {Phys. Rev. D},
	volume = {101},
	issue = {6},
	pages = {063001},
	numpages = {21},
	year = {2020},
	month = {Mar},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevD.101.063001},
	url = {https://link.aps.org/doi/10.1103/PhysRevD.101.063001}
}

@article{Abbar_2020,
	doi = {10.1088/1475-7516/2020/05/027},
	url = {https://dx.doi.org/10.1088/1475-7516/2020/05/027},
	year = {2020},
	month = {may},
	publisher = {},
	volume = {2020},
	number = {05},
	pages = {027},
	author = {Sajad Abbar},
	title = {Searching for  fast neutrino flavor conversion modes in core-collapse supernova simulations},
	journal = {Journal of Cosmology and Astroparticle Physics},
	abstract = {Neutrinos propagating in dense neutrino media such as those   in core-collapse supernovae can experience fast flavor conversions   on scales much shorter than those expected in vacuum.  It is   believed that a necessary condition for the occurrence of fast modes   is that the angular distributions of νe and ν̄e cross   each other. However, most of the state-of-the-art supernova   simulations do not provide such detailed angular information and   instead, consider only a few moments of neutrino angular   distributions.  We here propose an efficient method to use these   available few moments to search for fast modes in supernova   simulations.  Our method, which is based on searching for crossings   in the angular distributions, can work with any number of moments   provided by the simulation though a larger number of crossings can   be captured when higher moments are available.}
}

@article{PhysRevD.103.063013,
	title = {Fast neutrino flavor conversions in one-dimensional core-collapse supernova models with and without muon creation},
	author = {Capozzi, Francesco and Abbar, Sajad and Bollig, Robert and Janka, H.-Thomas},
	journal = {Phys. Rev. D},
	volume = {103},
	issue = {6},
	pages = {063013},
	numpages = {13},
	year = {2021},
	month = {Mar},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevD.103.063013},
	url = {https://link.aps.org/doi/10.1103/PhysRevD.103.063013}
}

@article{PhysRevD.104.083025,
	title = {Where, when, and why: Occurrence of fast-pairwise collective neutrino oscillation in three-dimensional core-collapse supernova models},
	author = {Nagakura, Hiroki and Burrows, Adam and Johns, Lucas and Fuller, George M.},
	journal = {Phys. Rev. D},
	volume = {104},
	issue = {8},
	pages = {083025},
	numpages = {17},
	year = {2021},
	month = {Oct},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevD.104.083025},
	url = {https://link.aps.org/doi/10.1103/PhysRevD.104.083025}
}

@article{Harada_2022,
	doi = {10.3847/1538-4357/ac38a0},
	url = {https://dx.doi.org/10.3847/1538-4357/ac38a0},
	year = {2022},
	month = {jan},
	publisher = {The American Astronomical Society},
	volume = {924},
	number = {2},
	pages = {109},
	author = {Akira Harada and Hiroki Nagakura},
	title = {Prospects of Fast Flavor Neutrino Conversion in Rotating Core-collapse Supernovae},
	journal = {The Astrophysical Journal},
	abstract = {There is mounting evidence that neutrinos undergo fast flavor conversion (FFC) in core-collapse supernova (CCSN). In this paper, we investigate the roles of stellar rotation on the occurrence of FFC by carrying out axisymmetric CCSN simulations with full Boltzmann neutrino transport. Our result suggests that electron neutrino lepton number (ELN) angular crossings, which are the necessary and sufficient condition to trigger FFC, preferably occur in the equatorial region for rotating CCSNe. By scrutinizing the neutrino–matter interaction and neutrino radiation field, we find some pieces of evidence that the stellar rotation facilitates the occurrence of FFC. The low-electron-fraction region in the post-shock layer expands by centrifugal force, enhancing the disparity of neutrino absorption between electron-type neutrinos (ν e) and their anti-particles (). This has a significant impact on the angular distribution of neutrinos in momentum space, in which ν e tends to be more isotropic than  consequently, ELN crossings emerge. The ELN crossing found in this study is clearly associated with rotation, which motivates further investigation on how the subsequent FFC influences explosion dynamics, nucleosynthesis, and neutrino signals in rotating CCSNe.}
}

@misc{https://doi.org/10.48550/arxiv.2206.01673,
	doi = {10.48550/ARXIV.2206.01673},
	
	url = {https://arxiv.org/abs/2206.01673},
	
	author = {Akaho, Ryuichiro and Harada, Akira and Nagakura, Hiroki and Iwakami, Wakana and Okawa, Hirotada and Furusawa, Shun and Matsufuru, Hideo and Sumiyoshi, Kohsuke and Yamada, Shoichi},
	
	keywords = {High Energy Astrophysical Phenomena (astro-ph.HE), FOS: Physical sciences, FOS: Physical sciences},
	
	title = {Protoneutron Star Convection Simulated with a New General Relativistic Boltzmann Neutrino Radiation-Hydrodynamics Code},
	
	publisher = {arXiv},
	
	year = {2022},
	
	copyright = {arXiv.org perpetual, non-exclusive license}
}




@article{PhysRevD.105.L101301,
	title = {Fast neutrino flavor instability and neutrino flavor lepton number crossings},
	author = {Morinaga, Taiki},
	journal = {Phys. Rev. D},
	volume = {105},
	issue = {10},
	pages = {L101301},
	numpages = {7},
	year = {2022},
	month = {May},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevD.105.L101301},
	url = {https://link.aps.org/doi/10.1103/PhysRevD.105.L101301}
}

@article{PhysRevD.107.083016,
	title = {Evolution of collisional neutrino flavor instabilities in spherically symmetric supernova models},
	author = {Xiong, Zewei and Wu, Meng-Ru and Mart\'{\i}nez-Pinedo, Gabriel and Fischer, Tobias and George, Manu and Lin, Chun-Yu and Johns, Lucas},
	journal = {Phys. Rev. D},
	volume = {107},
	issue = {8},
	pages = {083016},
	numpages = {20},
	year = {2023},
	month = {Apr},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevD.107.083016},
	url = {https://link.aps.org/doi/10.1103/PhysRevD.107.083016}
}

@article{PhysRevD.106.103031,
	title = {Neutrino fast flavor pendulum. II. Collisional damping},
	author = {Padilla-Gay, Ian and Tamborra, Irene and Raffelt, Georg G.},
	journal = {Phys. Rev. D},
	volume = {106},
	issue = {10},
	pages = {103031},
	numpages = {14},
	year = {2022},
	month = {Nov},
	publisher = {American Physical Society},
	doi = {10.1103/PhysRevD.106.103031},
	url = {https://link.aps.org/doi/10.1103/PhysRevD.106.103031}
}

